A Computationally Efficient EK-PMBM Filter for Bistatic mmWave Radio SLAM

Millimeter wave (mmWave) signals are useful for simultaneous localization and mapping (SLAM), due to their inherent geometric connection to the propagation environment and the propagation channel. To solve the SLAM problem, existing approaches rely on sigma-point or particle-based approximations, leading to high computational complexity, precluding real-time execution. We propose a novel low-complexity SLAM filter, based on the Poisson multi-Bernoulli mixture (PMBM) filter. It utilizes the extended Kalman (EK) first-order Taylor series based Gaussian approximation of the filtering distribution, and applies the track-oriented marginal multi-Bernoulli/Poisson (TOMB/P) algorithm to approximate the resulting PMBM as a Poisson multi-Bernoulli (PMB). The filter can account for different landmark types in radio SLAM and multiple data association hypotheses. Hence, it has an adjustable complexity/performance trade-off. Simulation results show that the developed SLAM filter can greatly reduce the computational cost, while it keeps the good performance of mapping and user state estimation.

==> 5G SLAM Using EKF-PMBM Filter-10/figure/Mapping.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor4}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor5}{rgb}{0,0,0}%
%\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[scale=0.5\linewidth/14cm]

\begin{axis}[%
width=6.028in,
height=2.009in,
at={(1.011in,2.014in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black},font=\Large},
xlabel={time step},
ymin=0,
ymax=30,
ymode=log,
ylabel style={font=\color{white!15!black},font=\Large},
ylabel={GOSPA distance [m]},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black,font=\Large}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	14.2815076877367\\
3	2.3608900273532\\
4	1.86958621565284\\
5	1.84516225700986\\
6	1.82471616888289\\
7	1.80336156394962\\
8	1.7231975543124\\
9	1.61050436045507\\
10	1.47896855142484\\
11	1.37991171497453\\
12	1.31889459290686\\
13	1.27495049797053\\
14	1.19680768138537\\
15	1.14339323656076\\
16	1.1069822560735\\
17	1.07043255541158\\
18	1.06273699026761\\
19	1.07699476815325\\
20	1.01864494481351\\
21	1.01429663711902\\
22	0.987275820613174\\
23	0.977165012472249\\
24	0.970575564873686\\
25	0.954105283182213\\
26	0.937263354530606\\
27	0.914164646178292\\
28	0.889351685504464\\
29	0.882919032535644\\
30	0.864814996967124\\
31	0.845338189598242\\
32	0.840632351631002\\
33	0.839442372262749\\
34	0.821967612893701\\
35	0.822412161423321\\
36	0.818034945505461\\
37	0.804953291279147\\
38	0.793965542821192\\
39	0.771694398539424\\
40	0.768904263367888\\
};
\addlegendentry{EK-PMB with $\gamma=10$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	14.61069038231981\\
3	2.19826893216357\\
4	2.38927711146112\\
5	2.13032718544272\\
6	1.94474480690431\\
7	1.97933545776544\\
8	1.77386528699347\\
9	1.6070924798458\\
10	1.50465853651786\\
11	1.41012643140318\\
12	1.38462024812301\\
13	1.32724705396888\\
14	1.27425011072173\\
15	1.22462386906783\\
16	1.19009341904979\\
17	1.14744627533138\\
18	1.15497554698392\\
19	1.14593421930795\\
20	1.11519096538842\\
21	1.07456747069257\\
22	1.07337321460548\\
23	1.07267204074422\\
24	1.05002654594153\\
25	1.04547118157319\\
26	1.03725850459664\\
27	1.02041671429084\\
28	1.02039692997218\\
29	1.01615805943879\\
30	1.00272215625274\\
31	0.992919026416869\\
32	0.983890333963561\\
33	0.966125092780923\\
34	0.960516638497756\\
35	0.947616401388431\\
36	0.936591470343951\\
37	0.913702551888904\\
38	0.905448113705986\\
39	0.89440618900431\\
40	0.891985854170959\\
};
\addlegendentry{EK-PMB with $\gamma=1$}

\addplot [color=mycolor5, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	14.4430664421268\\
3	2.01789900863084\\
4	1.75984004533113\\
5	1.78799162426577\\
6	1.77465707360237\\
7	1.79437876659862\\
8	1.59098915687467\\
9	1.44735577776576\\
10	1.32085506147508\\
11	1.2258595265087\\
12	1.17019999238103\\
13	1.09783332677967\\
14	1.074394284911376\\
15	0.982468827590847\\
16	0.974887982280766\\
17	0.959773489500317\\
18	0.912930092261505\\
19	0.896497976125273\\
20	0.915120828330582\\
21	0.905782483298157\\
22	0.884506918375166\\
23	0.852707193708485\\
24	0.848473909549964\\
25	0.830425134272638\\
26	0.830568921789277\\
27	0.811621905407414\\
28	0.800906983860668\\
29	0.788471541434889\\
30	0.766743547901116\\
31	0.761730214297476\\
32	0.766059131894456\\
33	0.778512660636621\\
34	0.75745049384834\\
35	0.741829362714729\\
36	0.740837984650758\\
37	0.732610289814097\\
38	0.731837948118093\\
39	0.725911880211699\\
40	0.730716498194207\\
};
\addlegendentry{EK-PMBM with $\gamma=10$}

\addplot [color=mycolor3, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	14.1803857775323\\
3	1.50812355513916\\
4	1.72277884814771\\
5	1.70831830238888\\
6	1.42406945946222\\
7	1.28794218772365\\
8	1.51416385612944\\
9	1.38268180621675\\
10	1.28371241249673\\
11	0.985651208176957\\
12	0.792895287022791\\
13	0.805932833188666\\
14	0.762946632949497\\
15	0.834267347792315\\
16	0.870129315123838\\
17	0.832483924910944\\
18	0.485210078939622\\
19	0.699260833372067\\
20	0.815166029897717\\
21	0.527902609866416\\
22	0.544960541854684\\
23	0.687760240404335\\
24	0.6526603300102\\
25	0.647619432477474\\
26	0.644751560978913\\
27	0.675031951875613\\
28	0.451323801265745\\
29	0.440465130885032\\
30	0.503362306760034\\
31	0.524372187058061\\
32	0.496057011411148\\
33	0.45095054468586\\
34	0.483495323333383\\
35	0.452424496806593\\
36	0.453239419863599\\
37	0.516779474802085\\
38	0.521324095236159\\
39	0.455142149449697\\
40	0.441573030627103\\
};
\addlegendentry{RBP-PMBM}

\addplot [color=mycolor4, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	21.9560780283641\\
3	7.54796845621767\\
4	7.76364840021301\\
5	5.45852711804379\\
6	4.40228915989216\\
7	4.69444305080753\\
8	3.81216841877973\\
9	3.12672216204169\\
10	3.140581393565\\
11	2.52032254937619\\
12	2.70488285522605\\
13	2.92636887563318\\
14	2.24577160977453\\
15	2.38945188087766\\
16	2.35094708498232\\
17	2.29582989022679\\
18	2.3143262790524\\
19	2.38298352397398\\
20	2.32916444927525\\
21	2.3270164183666\\
22	2.24105029379197\\
23	2.03313046552227\\
24	2.16430740470556\\
25	2.23666585164272\\
26	2.34738680895363\\
27	2.14219132977888\\
28	2.27943552257275\\
29	2.14384926234255\\
30	2.0016214396336\\
31	1.97579907931694\\
32	2.02628573567747\\
33	2.09604471631159\\
34	2.16139997443453\\
35	2.12140344376624\\
36	2.00159357359082\\
37	1.97686497667226\\
38	2.11211045066419\\
39	2.22050049651342\\
40	2.28902257403792\\
};
\addlegendentry{EK-PHD}

\end{axis}
\end{tikzpicture}%

==> 5G SLAM Using EKF-PMBM Filter-10/figure/Mapping_SP.tex <==
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor4}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor5}{rgb}{0,0,0}%
%\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
%
\begin{tikzpicture}[scale=0.5\linewidth/14cm]

\begin{axis}[%
width=6.028in,
height=2.009in,
at={(1.011in,2.014in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black},font=\Large},
xlabel={time step},
ymin=0,
ymax=30,
ymode=log,
ylabel style={font=\color{white!15!black},font=\Large},
ylabel={GOSPA distance [m]},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend pos=south west,
legend style={legend cell align=left, align=left, draw=white!15!black,font=\Large}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	24.4976104126054\\
3	24.4971726800625\\
4	24.4971726800625\\
5	24.4971726800625\\
6	24.4971726800625\\
7	24.4971726800625\\
8	20.0089606935208\\
9	20.006432279241\\
10	20.0043857271464\\
11	20.0046877977079\\
12	20.0051328095331\\
13	20.0048052713288\\
14	20.0048052713288\\
15	20.0048052713288\\
16	20.0048052713288\\
17	20.0048052713288\\
18	14.1602334840715\\
19	14.1542186548884\\
20	14.1514978309904\\
21	14.1509867039574\\
22	14.1502552456764\\
23	14.1500692849031\\
24	14.1500692849031\\
25	14.1500692849031\\
26	14.1500692849031\\
27	14.1500692849031\\
28	0.637075649071575\\
29	0.514538379627771\\
30	0.492985276726793\\
31	0.505962405801442\\
32	0.512787304142804\\
33	0.500015157159195\\
34	0.500015157159195\\
35	0.500015157159195\\
36	0.500015157159195\\
37	0.499934267880708\\
38	0.400520670101598\\
39	0.373244048861521\\
40	0.388478532031204\\
};
\addlegendentry{EK-PMB with $\gamma=10$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
  1	28.2842712474619\\
2	24.5064571081199\\
3	24.5013158304374\\
4	24.5013158304374\\
5	24.5013158304374\\
6	24.5013158304374\\
7	24.5013158304374\\
8	20.0150042013919\\
9	20.0131413894822\\
10	20.0119284496721\\
11	20.0109209274677\\
12	20.0125153216728\\
13	20.0126412925715\\
14	20.0126412925715\\
15	20.0126412925715\\
16	20.0126412925715\\
17	20.0126412925715\\
18	14.1735315745703\\
19	14.1704259925714\\
20	14.1647667323002\\
21	14.1606511961838\\
22	14.1606739238941\\
23	14.1609768707514\\
24	14.1609768707514\\
25	14.1609768707514\\
26	14.1609768707514\\
27	14.1609768707514\\
28	0.954050507105891\\
29	0.877818859544393\\
30	0.891589809903384\\
31	0.832712895320372\\
32	0.832155531989099\\
33	0.809488908553463\\
34	0.809488908553463\\
35	0.809488908553463\\
36	0.809488908553463\\
37	0.787730050703057\\
38	0.787730050703057\\
39	0.787730050703057\\
40	0.695162348415402\\
};
\addlegendentry{EK-PMB with $\gamma=1$}
\addplot [color=mycolor5, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	25.4450920267171\\
3	24.4976084237915\\
4	24.4976084237915\\
5	24.4976084237915\\
6	24.4976084237915\\
7	24.4976084237915\\
8	20.0116132309335\\
9	20.0075508016813\\
10	20.0055574989945\\
11	20.0056059010642\\
12	20.005459418142\\
13	20.0054723492403\\
14	20.0054723492403\\
15	20.0054723492403\\
16	20.0054723492403\\
17	20.0054723492403\\
18	14.1626121347146\\
19	14.153971121811\\
20	14.1532060110624\\
21	14.151508648118\\
22	14.1506709323724\\
23	14.150515747314\\
24	14.150515747314\\
25	14.150515747314\\
26	14.150515747314\\
27	14.150515747314\\
28	0.67158057945417\\
29	0.557490113070335\\
30	0.483406285972127\\
31	0.469356042946552\\
32	0.47006336947393\\
33	0.48282434207054\\
34	0.48282434207054\\
35	0.482824342070542\\
36	0.482824342070542\\
37	0.482824342070542\\
38	0.397302411898653\\
39	0.409103633320858\\
40	0.425969771023717\\
};
\addlegendentry{EK-PMBM with $\gamma=10$}

\addplot [color=mycolor3, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	24.4978826644068\\
3	24.4963723041687\\
4	24.4958725680683\\
5	24.4964735361943\\
6	24.4965770333216\\
7	24.4959647935387\\
8	20.0031058172215\\
9	20.0042873847625\\
10	20.0033419546934\\
11	20.0026327937978\\
12	20.0015246159575\\
13	20.0010730067171\\
14	20.0019723655925\\
15	20.0022157382861\\
16	20.0022080655755\\
17	20.0023120634136\\
18	14.1533124178684\\
19	14.1468694442103\\
20	14.1471326240372\\
21	14.1454474540427\\
22	14.1455653547584\\
23	14.1457198926402\\
24	14.1461038172215\\
25	14.1461496954345\\
26	14.1456867871757\\
27	14.145461478682\\
28	0.418497330109521\\
29	0.379603098644561\\
30	0.316375950268309\\
31	0.364009038554483\\
32	0.331511402470091\\
33	0.343940132150374\\
34	0.3274902107448\\
35	0.364743212592972\\
36	0.361051426457231\\
37	0.228475872945747\\
38	0.253156275080025\\
39	0.252748115195989\\
40	0.243095977559814\\
};
\addlegendentry{RBP-PMBM}

\addplot [color=mycolor4, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	28.2842712474619\\
2	24.5155827096825\\
3	24.5155827096825\\
4	24.5155827096825\\
5	24.5155827096825\\
6	24.5155827096825\\
7	24.5155827096825\\
8	20.015168159774\\
9	20.0098063880665\\
10	20.0086722683666\\
11	20.0028991727098\\
12	20.0042408656914\\
13	20.0042408656914\\
14	20.0042408656914\\
15	20.0042408656914\\
16	20.0042408656914\\
17	20.0042408656914\\
18	14.2721001040997\\
19	14.2568668319866\\
20	14.2196659194445\\
21	14.1660749947593\\
22	14.180384995944\\
23	14.180384995944\\
24	14.180384995944\\
25	14.180384995944\\
26	14.180384995944\\
27	14.180384995944\\
28	2.4299391434233\\
29  2.32327133095552\\
30	2.20451539580507\\
31	2.06375356005761\\
32	1.92752030833835\\
33	1.71314239090241\\
34	1.71314239090241\\
35	1.71314239090241\\
36	1.71314239090241\\
37	1.71314239090241\\
38	1.71314239090241\\
39	1.72934584634096\\
40	1.71436132982418\\
};
\addlegendentry{EK-PHD}

\end{axis}
\end{tikzpicture}%

==> 5G SLAM Using EKF-PMBM Filter-10/figure/pos_all.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0,0,0}
\begin{tikzpicture}[scale=0.5\linewidth/14cm]
\begin{axis}[%
width=6.028in,
height=2.009in,
at={(1.011in,2.014in)},
scale only axis,
xmin=0,
xmax=40,
xlabel style={font=\color{white!15!black},font=\Large},
xlabel={time step},
ymin=0,
ymax=0.5,
ymode=log,
ylabel style={font=\color{white!15!black},font=\Large},
ylabel={MAE of position [m]},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend pos=south west,
legend style={legend cell align=left, align=left, draw=white!15!black,font=\Large}
]
\addplot [color=mycolor1, line width=2.0pt]
  table[row sep=crcr]{%
1	0.244440000515429\\
2	0.205290109616914\\
3	0.221327431238034\\
4	0.20154519478018\\
5	0.202943276492121\\
6	0.179124525804273\\
7	0.186025990326865\\
8	0.1756059435913\\
9	0.19464951154528\\
10	0.189741132585282\\
11	0.19658152553044\\
12	0.197150248032116\\
13	0.185864478447547\\
14	0.188395916284782\\
15	0.200622668741351\\
16	0.19504336252507\\
17	0.196381738635173\\
18	0.179452460992472\\
19	0.19176767720128\\
20	0.198168058773379\\
21	0.162096670965647\\
22	0.174451459215614\\
23	0.18573836500874\\
24	0.167517667698087\\
25	0.157104401030743\\
26	0.157742915583309\\
27	0.168879731931658\\
28	0.134116529748964\\
29	0.152888885028984\\
30	0.121416765229553\\
31	0.123966301628717\\
32	0.133049006821639\\
33	0.134105464433002\\
34	0.135649616295674\\
35	0.13015730116451\\
36	0.115443192691654\\
37	0.129475338390738\\
38	0.103662606780303\\
39	0.118698337722304\\
40	0.114061248516018\\
};
\addlegendentry{EK-PMB with $\gamma=10$}

\addplot [color=mycolor2, line width=2.0pt]
  table[row sep=crcr]{%
1	0.265317869343472\\
2	0.230984376246761\\
3	0.22435271738992\\
4	0.224085023516584\\
5	0.234038625941373\\
6	0.223092554229443\\
7	0.232292948536294\\
8	0.236714782189392\\
9	0.242408079500099\\
10	0.250125736338311\\
11	0.235602986511245\\
12	0.230882521233124\\
13	0.231187327301165\\
14	0.234776745355362\\
15	0.22369677633864\\
16	0.224762548722461\\
17	0.223297755909402\\
18	0.199290920701279\\
19	0.199315186447989\\
20	0.211189005346257\\
21	0.17655234956308\\
22	0.194927789567335\\
23	0.180840766546827\\
24	0.184922075140926\\
25	0.204704279483\\
26	0.189259891156599\\
27	0.183633852374608\\
28	0.173067604130544\\
29	0.183859808574596\\
30	0.17642658882136\\
31	0.165277115022679\\
32	0.166672371123579\\
33	0.152567810431965\\
34	0.158587063664491\\
35	0.148807240973771\\
36	0.155970933466099\\
37	0.147246195342202\\
38	0.143565202466063\\
39	0.149149077301643\\
40	0.146044865766664\\
};
\addlegendentry{EK-PMB with $\gamma=1$}
\addplot [color=mycolor5, line width=2.0pt]
  table[row sep=crcr]{%
1	0.24605584179777\\
2	0.191761104686047\\
3	0.193217839853405\\
4	0.194972113416861\\
5	0.181436573165629\\
6	0.175147705869261\\
7	0.187713102612364\\
8	0.184073911782016\\
9	0.176021547540539\\
10	0.178433147829893\\
11	0.186755250664017\\
12	0.169098406892002\\
13	0.168662928309646\\
14	0.163194373895529\\
15	0.169637249546059\\
16	0.161854722109028\\
17	0.170459974512376\\
18	0.168126061655579\\
19	0.167546359465238\\
20	0.154388035389341\\
21	0.167374421381603\\
22	0.163537875781349\\
23	0.145595481382161\\
24	0.177057198993474\\
25	0.171247316862037\\
26	0.165907069742891\\
27	0.158795802366045\\
28	0.13974798660183\\
29	0.155828005997876\\
30	0.141490921119289\\
31	0.140516028676828\\
32	0.122100387651142\\
33	0.137107964680661\\
34	0.130957847896183\\
35	0.1302837188732\\
36	0.123923596346672\\
37	0.115529269277191\\
38	0.122036736495554\\
39	0.123884167685235\\
40	0.115714518558786\\
};
\addlegendentry{EK-PMBM with $\gamma=10$}
\addplot [color=mycolor1, dashed, line width=2.0pt]
  table[row sep=crcr]{%
1	0.261632147788967\\
2	0.182320520119313\\
3	0.0654916428932192\\
4	0.0626561610113271\\
5	0.163902515881458\\
6	0.155808702454556\\
7	0.0692633865181821\\
8	0.125809266198656\\
9	0.0661441157130687\\
10	0.0673257264538966\\
11	0.0885092421455029\\
12	0.148238387141577\\
13	0.0264424822400462\\
14	0.0493307701488435\\
15	0.0301654955207687\\
16	0.121010022694884\\
17	0.0593894327667528\\
18	0.0597602435752879\\
19	0.0246716097500183\\
20	0.0385881766524143\\
21	0.10559105712871\\
22	0.125176580847014\\
23	0.111824633010669\\
24	0.0947032635089333\\
25	0.13131443512261\\
26	0.0829528082518841\\
27	0.182097789801394\\
28	0.0578183869993756\\
29	0.116933449465601\\
30	0.144749461428704\\
31	0.126943161133796\\
32	0.235637919801675\\
33	0.101893869058206\\
34	0.0324044300803358\\
35	0.0236404068128193\\
36	0.048194753766114\\
37	0.0648670013227506\\
38	0.0254005396933729\\
39	0.0579483957883275\\
40	0.0504030792397435\\
};
\addlegendentry{RBP-PMBM}
\addplot [color=mycolor2, line width=2.0pt, dashed]
  table[row sep=crcr]{%
1	0.253872309690221\\
2	0.286497782391864\\
3	0.260549355682194\\
4	0.31290178537244\\
5	0.241411775516621\\
6	0.313526155225513\\
7	0.285320100650327\\
8	0.266907101227159\\
9	0.319957166736913\\
10	0.260089706393788\\
11	0.266839977504255\\
12	0.257382662007393\\
13	0.264675740815087\\
14	0.248587376882623\\
15	0.25251865086705\\
16	0.248429780944707\\
17	0.292761299646314\\
18	0.264155482149693\\
19	0.243003655326713\\
20	0.272297839618443\\
21	0.247111310883289\\
22	0.225993574771313\\
23	0.247302216595056\\
24	0.186159102498665\\
25	0.244304959270289\\
26	0.177445404898966\\
27	0.230979511641287\\
28	0.181388395138674\\
29	0.266528825482145\\
30	0.18004473555537\\
31	0.173193737817831\\
32	0.175620053629193\\
33	0.186055582628016\\
34	0.211009745836464\\
35	0.174413915015655\\
36	0.188013466107511\\
37	0.15083920592114\\
38	0.169297676272941\\
39	0.178528251701103\\
40	0.173107178268878\\
};
\addlegendentry{EK-PHD}
\end{axis}

\end{tikzpicture}%

==> 5G SLAM Using EKF-PMBM Filter-10/figure/pos_bar.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}
\definecolor{mycolor5}{rgb}{0,0,0}%
%
\begin{tikzpicture}[scale=0.6\linewidth/14cm]

\begin{axis}[%
width=3.842in,
height=1.281in,
at={(3.465in,2.378in)},
scale only axis,
bar shift auto,
xmin=0.5,
xmax=3.5,
xtick={1,2,3},
xticklabels={{position},{heading},{clock bias}},
ymin=0,
ymax=0.3,
ylabel style={font=\color{white!15!black}},
ylabel={RMSE of state [m], [deg], [m]},
axis background/.style={fill=white},
legend style={at={(-0.15,1)}, anchor=north east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot[ybar, bar width=0.145, fill=mycolor1, draw=black, area legend] table[row sep=crcr] {%
1	0.1663\\
2	0.1362\\
3	0.0898\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.5	0\\
3.5	0\\
};
\addlegendentry{EK-PMB with $\gamma=10$}

\addplot[ybar, bar width=0.145, fill=mycolor2, draw=black, area legend] table[row sep=crcr] {%
1	0.1979\\
2	0.1693\\
3	0.1016\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.5	0\\
3.5	0\\
};
\addlegendentry{EK-PMB with $\gamma=1$}

\addplot[ybar, bar width=0.145, fill=mycolor5, draw=black, area legend] table[row sep=crcr] {%
1	0.1604\\
2	0.1339\\
3	0.0857\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.5	0\\
3.5	0\\
};
\addlegendentry{EK-PMBM with $\gamma=10$}

\addplot[ybar, bar width=0.145, fill=mycolor3, draw=black, area legend] table[row sep=crcr] {%
1	0.1477\\
2	0.1048\\
3	0.0753\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.5	0\\
3.5	0\\
};
\addlegendentry{RBP-PMBM}

\addplot[ybar, bar width=0.145, fill=mycolor4, draw=black, area legend] table[row sep=crcr] {%
1	0.2542\\
2	0.2078\\
3	0.1423\\
};
\addplot[forget plot, color=white!15!black] table[row sep=crcr] {%
0.5	0\\
3.5	0\\
};
\addlegendentry{EK-PHD}

\end{axis}
\end{tikzpicture}%

==> 5G SLAM Using EKF-PMBM Filter-10/figure/theenv.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}[scale=0.8\linewidth/14cm]

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=-200,
xmax=200,
tick align=outside,
xlabel style={font=\color{white!15!black}},
xlabel={X [m]},
ymin=-200,
ymax=200,
ylabel style={font=\color{white!15!black}},
ylabel={Y [m]},
zmin=0,
zmax=40,
zlabel style={font=\color{white!15!black}},
zlabel={Z [m]},
view={75}{85},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
axis z line*=left,
xmajorgrids,
ymajorgrids,
zmajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot3 [ycomb, color=black, mark=triangle, mark options={solid, black}]
 table[row sep=crcr] {%
0	0	40\\
};
 \addlegendentry{BS}

\node[right, align=left]
at (axis cs:0,3,38) {(0,0,40)};
\addplot3 [color=mycolor1, line width=1.0pt]
 table[row sep=crcr] {%
70.7285	0	0\\
70.6611821401524	3.08513383926917	0\\
70.459356703982	6.16439495092774	0\\
70.1234078776776	9.23192178643592	0\\
69.653975158924	12.2818751341155	0\\
69.0519521395822	15.3084492344211	0\\
68.3184848046864	18.3058828315336	0\\
67.454969350996	21.268470140238	0\\
66.4630495292561	24.1905717072096	0\\
65.3446135152245	27.0666251460343	0\\
64.1017903154217	29.8911557255271	0\\
62.7369457144459	32.6587867911941	0\\
61.2526777715677	35.36425	0\\
59.6518118751767	38.0023953489583	0\\
57.937395364494	40.568200978455	0\\
56.1126917287886	43.0567827316433	0\\
54.1811743951406	45.4634034517144	0\\
52.1465201165749	47.7834819993442	0\\
50.0126019731527	50.0126019731527	0\\
47.7834819993442	52.1465201165748	0\\
45.4634034517144	54.1811743951406	0\\
43.0567827316433	56.1126917287886	0\\
40.568200978455	57.937395364494	0\\
38.0023953489583	59.6518118751767	0\\
35.36425	61.2526777715677	0\\
32.6587867911941	62.7369457144458	0\\
29.8911557255271	64.1017903154217	0\\
27.0666251460343	65.3446135152245	0\\
24.1905717072096	66.4630495292561	0\\
21.268470140238	67.454969350996	0\\
18.3058828315336	68.3184848046864	0\\
15.3084492344211	69.0519521395822	0\\
12.2818751341155	69.653975158924	0\\
9.23192178643593	70.1234078776776	0\\
6.16439495092775	70.459356703982	0\\
3.08513383926917	70.6611821401524	0\\
4.33087155667468e-15	70.7285	0\\
-3.08513383926916	70.6611821401524	0\\
-6.16439495092773	70.459356703982	0\\
-9.23192178643592	70.1234078776776	0\\
-12.2818751341155	69.653975158924	0\\
-15.3084492344211	69.0519521395822	0\\
-18.3058828315336	68.3184848046864	0\\
-21.268470140238	67.454969350996	0\\
-24.1905717072096	66.4630495292561	0\\
-27.0666251460342	65.3446135152245	0\\
-29.891155725527	64.1017903154217	0\\
-32.6587867911941	62.7369457144459	0\\
-35.36425	61.2526777715677	0\\
-38.0023953489583	59.6518118751767	0\\
-40.5682009784549	57.937395364494	0\\
-43.0567827316433	56.1126917287886	0\\
-45.4634034517144	54.1811743951406	0\\
-47.7834819993442	52.1465201165749	0\\
-50.0126019731527	50.0126019731527	0\\
-52.1465201165748	47.7834819993442	0\\
-54.1811743951406	45.4634034517144	0\\
-56.1126917287886	43.0567827316433	0\\
-57.9373953644939	40.568200978455	0\\
-59.6518118751767	38.0023953489583	0\\
-61.2526777715677	35.36425	0\\
-62.7369457144459	32.6587867911941	0\\
-64.1017903154217	29.8911557255271	0\\
-65.3446135152245	27.0666251460343	0\\
-66.4630495292561	24.1905717072096	0\\
-67.454969350996	21.268470140238	0\\
-68.3184848046864	18.3058828315337	0\\
-69.0519521395822	15.3084492344211	0\\
-69.653975158924	12.2818751341155	0\\
-70.1234078776776	9.23192178643592	0\\
-70.459356703982	6.16439495092774	0\\
-70.6611821401524	3.08513383926917	0\\
-70.7285	8.66174311334936e-15	0\\
-70.6611821401524	-3.08513383926915	0\\
-70.459356703982	-6.16439495092772	0\\
-70.1234078776776	-9.2319217864359	0\\
-69.653975158924	-12.2818751341155	0\\
-69.0519521395822	-15.3084492344211	0\\
-68.3184848046864	-18.3058828315336	0\\
-67.454969350996	-21.268470140238	0\\
-66.4630495292561	-24.1905717072096	0\\
-65.3446135152246	-27.0666251460342	0\\
-64.1017903154217	-29.891155725527	0\\
-62.7369457144459	-32.6587867911941	0\\
-61.2526777715677	-35.36425	0\\
-59.6518118751767	-38.0023953489583	0\\
-57.937395364494	-40.568200978455	0\\
-56.1126917287886	-43.0567827316433	0\\
-54.1811743951406	-45.4634034517144	0\\
-52.1465201165749	-47.7834819993442	0\\
-50.0126019731527	-50.0126019731527	0\\
-47.7834819993442	-52.1465201165748	0\\
-45.4634034517144	-54.1811743951406	0\\
-43.0567827316433	-56.1126917287886	0\\
-40.5682009784549	-57.937395364494	0\\
-38.0023953489584	-59.6518118751767	0\\
-35.36425	-61.2526777715677	0\\
-32.6587867911941	-62.7369457144458	0\\
-29.891155725527	-64.1017903154217	0\\
-27.0666251460343	-65.3446135152245	0\\
-24.1905717072095	-66.4630495292561	0\\
-21.268470140238	-67.454969350996	0\\
-18.3058828315336	-68.3184848046864	0\\
-15.3084492344211	-69.0519521395822	0\\
-12.2818751341155	-69.653975158924	0\\
-9.23192178643592	-70.1234078776776	0\\
-6.16439495092775	-70.459356703982	0\\
-3.08513383926918	-70.6611821401524	0\\
-1.2992614670024e-14	-70.7285	0\\
3.08513383926915	-70.6611821401524	0\\
6.16439495092772	-70.459356703982	0\\
9.2319217864359	-70.1234078776776	0\\
12.2818751341155	-69.653975158924	0\\
15.3084492344211	-69.0519521395822	0\\
18.3058828315336	-68.3184848046864	0\\
21.268470140238	-67.454969350996	0\\
24.1905717072095	-66.4630495292561	0\\
27.0666251460343	-65.3446135152245	0\\
29.891155725527	-64.1017903154217	0\\
32.6587867911941	-62.7369457144458	0\\
35.36425	-61.2526777715677	0\\
38.0023953489583	-59.6518118751767	0\\
40.568200978455	-57.937395364494	0\\
43.0567827316433	-56.1126917287886	0\\
45.4634034517144	-54.1811743951406	0\\
47.7834819993442	-52.1465201165749	0\\
50.0126019731527	-50.0126019731527	0\\
52.1465201165748	-47.7834819993442	0\\
54.1811743951406	-45.4634034517144	0\\
56.1126917287886	-43.0567827316433	0\\
57.9373953644939	-40.568200978455	0\\
59.6518118751767	-38.0023953489584	0\\
61.2526777715676	-35.36425	0\\
62.7369457144458	-32.6587867911941	0\\
64.1017903154217	-29.8911557255271	0\\
65.3446135152245	-27.0666251460343	0\\
66.4630495292561	-24.1905717072095	0\\
67.454969350996	-21.268470140238	0\\
68.3184848046864	-18.3058828315336	0\\
69.0519521395822	-15.3084492344211	0\\
69.653975158924	-12.2818751341155	0\\
70.1234078776776	-9.23192178643593	0\\
70.459356703982	-6.16439495092775	0\\
70.6611821401524	-3.08513383926918	0\\
70.7285	-1.73234862266987e-14	0\\
};
 \addlegendentry{trail}

\addplot3 [ycomb, color=blue, mark=asterisk, mark options={solid, blue}]
 table[row sep=crcr] {%
-200	0	40\\
200	0	40\\
0	-200	40\\
0	200	40\\
};
 \addlegendentry{VAs}

\node[right, align=left]
at (axis cs:-200,0,40) {(-200,0,40)};
\node[right, align=left]
at (axis cs:200,0,40) {(200,0,40)};
\node[right, align=left]
at (axis cs:0,200,40) {(0,200,40)};
\node[right, align=left]
at (axis cs:0,-200,40) {(0,-200,40)};
\node[right, align=left]
at (axis cs:30,30.729,0) {r=70.7285};
\addplot3 [ycomb, color=red, mark=asterisk, mark options={solid, red}]
 table[row sep=crcr] {%
-99	0	10\\
99	0	10\\
0	-99	10\\
0	99	10\\
};
 \addlegendentry{SPs}

\node[right, align=left]
at (axis cs:-96,0,10) {(-99,0,10)};
\node[right, align=left]
at (axis cs:96,0,10) {(99,0,10)};
\node[right, align=left]
at (axis cs:0,96,10) {(0,99,10)};
\node[right, align=left]
at (axis cs:0,-96,10) {(0,-99,10)};
\addplot3 [ycomb, color=blue, mark=square, mark options={solid, blue}]
 table[row sep=crcr] {%
70.7285	0	0\\
};
 \addlegendentry{Initial location of v1}

\end{axis}
\end{tikzpicture}%

==> figure/theenv.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%
%
\begin{tikzpicture}[scale=0.8\linewidth/14cm]

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmin=-200,
xmax=200,
tick align=outside,
xlabel style={font=\color{white!15!black}},
xlabel={X [m]},
ymin=-200,
ymax=200,
ylabel style={font=\color{white!15!black}},
ylabel={Y [m]},
zmin=0,
zmax=40,
zlabel style={font=\color{white!15!black}},
zlabel={Z [m]},
view={75}{85},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
axis z line*=left,
xmajorgrids,
ymajorgrids,
zmajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot3 [ycomb, color=black, mark=triangle, mark options={solid, black}]
 table[row sep=crcr] {%
0	0	40\\
};
 \addlegendentry{BS}

\node[right, align=left]
at (axis cs:0,3,38) {(0,0,40)};
\addplot3 [color=mycolor1, line width=1.0pt]
 table[row sep=crcr] {%
70.7285	0	0\\
70.6611821401524	3.08513383926917	0\\
70.459356703982	6.16439495092774	0\\
70.1234078776776	9.23192178643592	0\\
69.653975158924	12.2818751341155	0\\
69.0519521395822	15.3084492344211	0\\
68.3184848046864	18.3058828315336	0\\
67.454969350996	21.268470140238	0\\
66.4630495292561	24.1905717072096	0\\
65.3446135152245	27.0666251460343	0\\
64.1017903154217	29.8911557255271	0\\
62.7369457144459	32.6587867911941	0\\
61.2526777715677	35.36425	0\\
59.6518118751767	38.0023953489583	0\\
57.937395364494	40.568200978455	0\\
56.1126917287886	43.0567827316433	0\\
54.1811743951406	45.4634034517144	0\\
52.1465201165749	47.7834819993442	0\\
50.0126019731527	50.0126019731527	0\\
47.7834819993442	52.1465201165748	0\\
45.4634034517144	54.1811743951406	0\\
43.0567827316433	56.1126917287886	0\\
40.568200978455	57.937395364494	0\\
38.0023953489583	59.6518118751767	0\\
35.36425	61.2526777715677	0\\
32.6587867911941	62.7369457144458	0\\
29.8911557255271	64.1017903154217	0\\
27.0666251460343	65.3446135152245	0\\
24.1905717072096	66.4630495292561	0\\
21.268470140238	67.454969350996	0\\
18.3058828315336	68.3184848046864	0\\
15.3084492344211	69.0519521395822	0\\
12.2818751341155	69.653975158924	0\\
9.23192178643593	70.1234078776776	0\\
6.16439495092775	70.459356703982	0\\
3.08513383926917	70.6611821401524	0\\
4.33087155667468e-15	70.7285	0\\
-3.08513383926916	70.6611821401524	0\\
-6.16439495092773	70.459356703982	0\\
-9.23192178643592	70.1234078776776	0\\
-12.2818751341155	69.653975158924	0\\
-15.3084492344211	69.0519521395822	0\\
-18.3058828315336	68.3184848046864	0\\
-21.268470140238	67.454969350996	0\\
-24.1905717072096	66.4630495292561	0\\
-27.0666251460342	65.3446135152245	0\\
-29.891155725527	64.1017903154217	0\\
-32.6587867911941	62.7369457144459	0\\
-35.36425	61.2526777715677	0\\
-38.0023953489583	59.6518118751767	0\\
-40.5682009784549	57.937395364494	0\\
-43.0567827316433	56.1126917287886	0\\
-45.4634034517144	54.1811743951406	0\\
-47.7834819993442	52.1465201165749	0\\
-50.0126019731527	50.0126019731527	0\\
-52.1465201165748	47.7834819993442	0\\
-54.1811743951406	45.4634034517144	0\\
-56.1126917287886	43.0567827316433	0\\
-57.9373953644939	40.568200978455	0\\
-59.6518118751767	38.0023953489583	0\\
-61.2526777715677	35.36425	0\\
-62.7369457144459	32.6587867911941	0\\
-64.1017903154217	29.8911557255271	0\\
-65.3446135152245	27.0666251460343	0\\
-66.4630495292561	24.1905717072096	0\\
-67.454969350996	21.268470140238	0\\
-68.3184848046864	18.3058828315337	0\\
-69.0519521395822	15.3084492344211	0\\
-69.653975158924	12.2818751341155	0\\
-70.1234078776776	9.23192178643592	0\\
-70.459356703982	6.16439495092774	0\\
-70.6611821401524	3.08513383926917	0\\
-70.7285	8.66174311334936e-15	0\\
-70.6611821401524	-3.08513383926915	0\\
-70.459356703982	-6.16439495092772	0\\
-70.1234078776776	-9.2319217864359	0\\
-69.653975158924	-12.2818751341155	0\\
-69.0519521395822	-15.3084492344211	0\\
-68.3184848046864	-18.3058828315336	0\\
-67.454969350996	-21.268470140238	0\\
-66.4630495292561	-24.1905717072096	0\\
-65.3446135152246	-27.0666251460342	0\\
-64.1017903154217	-29.891155725527	0\\
-62.7369457144459	-32.6587867911941	0\\
-61.2526777715677	-35.36425	0\\
-59.6518118751767	-38.0023953489583	0\\
-57.937395364494	-40.568200978455	0\\
-56.1126917287886	-43.0567827316433	0\\
-54.1811743951406	-45.4634034517144	0\\
-52.1465201165749	-47.7834819993442	0\\
-50.0126019731527	-50.0126019731527	0\\
-47.7834819993442	-52.1465201165748	0\\
-45.4634034517144	-54.1811743951406	0\\
-43.0567827316433	-56.1126917287886	0\\
-40.5682009784549	-57.937395364494	0\\
-38.0023953489584	-59.6518118751767	0\\
-35.36425	-61.2526777715677	0\\
-32.6587867911941	-62.7369457144458	0\\
-29.891155725527	-64.1017903154217	0\\
-27.0666251460343	-65.3446135152245	0\\
-24.1905717072095	-66.4630495292561	0\\
-21.268470140238	-67.454969350996	0\\
-18.3058828315336	-68.3184848046864	0\\
-15.3084492344211	-69.0519521395822	0\\
-12.2818751341155	-69.653975158924	0\\
-9.23192178643592	-70.1234078776776	0\\
-6.16439495092775	-70.459356703982	0\\
-3.08513383926918	-70.6611821401524	0\\
-1.2992614670024e-14	-70.7285	0\\
3.08513383926915	-70.6611821401524	0\\
6.16439495092772	-70.459356703982	0\\
9.2319217864359	-70.1234078776776	0\\
12.2818751341155	-69.653975158924	0\\
15.3084492344211	-69.0519521395822	0\\
18.3058828315336	-68.3184848046864	0\\
21.268470140238	-67.454969350996	0\\
24.1905717072095	-66.4630495292561	0\\
27.0666251460343	-65.3446135152245	0\\
29.891155725527	-64.1017903154217	0\\
32.6587867911941	-62.7369457144458	0\\
35.36425	-61.2526777715677	0\\
38.0023953489583	-59.6518118751767	0\\
40.568200978455	-57.937395364494	0\\
43.0567827316433	-56.1126917287886	0\\
45.4634034517144	-54.1811743951406	0\\
47.7834819993442	-52.1465201165749	0\\
50.0126019731527	-50.0126019731527	0\\
52.1465201165748	-47.7834819993442	0\\
54.1811743951406	-45.4634034517144	0\\
56.1126917287886	-43.0567827316433	0\\
57.9373953644939	-40.568200978455	0\\
59.6518118751767	-38.0023953489584	0\\
61.2526777715676	-35.36425	0\\
62.7369457144458	-32.6587867911941	0\\
64.1017903154217	-29.8911557255271	0\\
65.3446135152245	-27.0666251460343	0\\
66.4630495292561	-24.1905717072095	0\\
67.454969350996	-21.268470140238	0\\
68.3184848046864	-18.3058828315336	0\\
69.0519521395822	-15.3084492344211	0\\
69.653975158924	-12.2818751341155	0\\
70.1234078776776	-9.23192178643593	0\\
70.459356703982	-6.16439495092775	0\\
70.6611821401524	-3.08513383926918	0\\
70.7285	-1.73234862266987e-14	0\\
};
 \addlegendentry{trail}

\addplot3 [ycomb, color=blue, mark=asterisk, mark options={solid, blue}]
 table[row sep=crcr] {%
-200	0	40\\
200	0	40\\
0	-200	40\\
0	200	40\\
};
 \addlegendentry{VAs}

\node[right, align=left]
at (axis cs:-200,0,40) {(-200,0,40)};
\node[right, align=left]
at (axis cs:200,0,40) {(200,0,40)};
\node[right, align=left]
at (axis cs:0,200,40) {(0,200,40)};
\node[right, align=left]
at (axis cs:0,-200,40) {(0,-200,40)};
\node[right, align=left]
at (axis cs:30,30.729,0) {r=70.7285};
\addplot3 [ycomb, color=red, mark=asterisk, mark options={solid, red}]
 table[row sep=crcr] {%
-99	0	10\\
99	0	10\\
0	-99	10\\
0	99	10\\
};
 \addlegendentry{SPs}

\node[right, align=left]
at (axis cs:-96,0,10) {(-99,0,10)};
\node[right, align=left]
at (axis cs:96,0,10) {(99,0,10)};
\node[right, align=left]
at (axis cs:0,96,10) {(0,99,10)};
\node[right, align=left]
at (axis cs:0,-96,10) {(0,-99,10)};
\addplot3 [ycomb, color=blue, mark=square, mark options={solid, blue}]
 table[row sep=crcr] {%
70.7285	0	0\\
};
 \addlegendentry{Initial location of v1}

\end{axis}
\end{tikzpicture}%
